Real-time Cosmology with High Precision Spectroscopy and Astrometry

Breakthroughs in physics and astrophysics are often driven by technological advances, with the recent detection of gravitational waves being one such example. This white paper focuses upon how improved astrometric and spectroscopic measurements from a new generation of precise, accurate, and stable astronomical instrumentation can address two of the fundamental mysteries of our time -- dark energy and dark matter -- and probe the nature of spacetime. Instrumentation is now on the cusp of enabling new cosmological measurements based on redshifts (cosmic redshift drift) and extremely precise time-series measurements of accelerations, astrophysical source positions (astrometry), and angles (cosmic parallax). These allow tests of the fundamental framework of the universe (the Friedmann equations of general relativity and whether cosmic expansion is physically accelerating) and its contents (dark energy evolution and dark matter behavior), while also anchoring the cosmic distance scale ($H_0$).

==> HighPrecision_Revised.tex <==

%\documentclass{article}
%\usepackage[utf8]{inputenc} 
%\usepackage{amssymb}
%\usepackage{amsmath}

%\begin{document}
	
\subsection{High Precision Cosmology Through Cosmological Parallax}

Our motion with respect to the Cosmic Microwave Background (CMB) 
results in positional changes with time for extragalactic sources that depend 
on the transverse co-moving distance. Thus our space motion provides 
a baseline 80 times larger per year than that provided by the Earth's 
annular motion. Since our CMB velocity is both an absolute reference and 
known to better than 1\% the precision, astrometry of quasars can provide a new 
measurement of the Hubble Constant that is independent of the traditional 
methods. Thus, it offers a means to directly address the current tension 
between empirical bootstrapped measurements and the value inferred from 
the consensus standard model (e.g., Freedman 2017). 

The cosmological parallactic distance is related to the transverse co-moving 
distance ($D_M$). Since this secular measure involves a transverse velocity 
it has a different dependence with redshift than does an angular size measure such as 
BAO due to time dilation with redshift. The three standard measures of cosmological 
distance are related through the transverse co-moving distance ($D_M$) but with differing 
dependencies on the cosmological parameters and the Dark Energy equation of state 
(e.g., Weinberg 1971; Hogg 2000; Peebles 2000; Huterer \& Turner 2001). 

The luminosity and angular size distances are well known but the measurement of cosmological 
parallax is less so. Apparent angular positional shifts ($\theta$) due to our motion 
through space can be used to computed the cosmological parallax and the 
transverse co-moving distance: 
$D_P = 1/\theta$. Being purely geometrical minimizes most of the systematics associated with measuring cosmological geometry. The measurement of cosmological parallax would thus 
provide a new measure of the cosmological parameters and the Dark Energy 
equation of state that is independent of the methods that have been used 
to date [SN Ia and Baryon Acoustic Oscillations (BAO), e.g., Alam et al. 2020]. 

\subsection{Limitations of the GAIA Astrometric Satellite}

At cosmologically interesting redshifts ($z \sim 1$), the secular parallax for 
the consensus cosmology is approximately $10^{-6}$ arc seconds over ten years 
of our motion. The relatively bright flux limit of the GAIA satellite limits 
precision astrometry to the nearest galactic nuclei and quasars. Furthermore, the presence 
of systematic errors at the few $10^{-6}$ arcsec level limits any parallax measurement via 
ensemble averaging of fainter quasar populations (GAIA Mission Science Performance). 
Various space-based astrometric 
missions have been proposed that may ultimately result in a measurement of cosmological 
parallax using fainter quasars (see Ding \& Croft 2009 for an assessment) but none of these have 
been funded. Similarly, a global array of radio telescopes, such as ngVLA, may ultimately 
achieve the required astrometric precision using a 
sample of compact radio loud quasars (e.g., Paine et al. 2020). The ngVLA was 
endorsed by the Astro 2020 Decadal Survey and received a 2nd priority ranking. 
If funded, it could potentially begin science operations in 2035 and be applied to the 
measurement of cosmological parallax.

\subsection{Precision Cosmology via Astrometry of Gravitationally Lensed Galaxies and Quasars}

An alternative to space-based astrometry and global interferometry is provided by the next 
generation of extremely large telescopes (ELTs) equipped with adaptive optics. These 
telescopes will provide an unprecedented astrometric precision. US participation in two 
of the ELTs currently under development, the Giant Magellan and Thirty Meter Telescopes, 
was ranked the highest priority of Astro 2020 Decadal Review. Most of their funding is 
already in place such that their technical development is underway. Their fields of view will be 
narrow precluding an all sky astrometric survey. However, their narrow-field performance 
still offer distinct advantages for the measurement of cosmological parallax. 
In particular, the gravitational lensing of quasars by foreground galaxies 
magnifies the differential positional shifts between the foreground lens and 
the background source $\sim 5\times$ as our line-of-sight changes with time. Particular 
attention is being paid to the long term astrometric stability of the ELTs. Simulations to 
date imply astrometric precisions of $3 \times 10^{-6}$ arcsec (e.g., Cameron et al. 2009) 
suggesting that these ELTs will provide a measurement of cosmological parallax and the 
transverse co-moving distance for the first time. 

\subsection{Synergies with the Rubin and Roman Surveys and the Path Forward}

The Rubin and Roman surveys are predicted to discover several thousand lensed quasars 
and compact galaxies (Oguri \& Marshall 2010). The angular magnifications in a typical lensed 
systems is about 5x bringing the signal up to a level measurable with the ELTs. Recent simulations 
(Pierce \& McGough, in preparation) have demonstrated that the astrometry of a single system 
with the ELTs will provide a several sigma detection of the cosmological parallax signal. Those 
simulations show that  ELT astrometry of only about 300 systems around the sky would provide 
constraints on the cosmological parameters and the Dark Energy equation of 
state that are comparable to those currently from BAO and SNIa. Thus, the measurement of 
cosmological parallax over the next few decades appears both feasible and inevitable. 

The ELTs promise to provide truly ground breaking capabilities for a number of research 
areas. As a result, the available time on the ELTs will be highly competed. 
We propose two strategies for a precision ELT measurement of the cosmological parallax and 
a corresponding constraint on the transverse co-moving distance:

$\bullet$ {\bf Rely on Public ELT time:} Lensed quasars are relatively bright and our simulations 
imply that precision astrometry could be acquired for about 10 systems/night of ELT time. 
Thus precision astrometry for a sample of 300 systems would require approximately 30 nights of 
telescope time for each epoch. The current estimate of the operational cost for the ELTs time is 
\$1.5M/night. This may limit the measurement of cosmological parallax to a minimal sample measured at 
two 
epochs.

$\bullet$ {\bf Construct Dedicated ELTs:} The sample of lensed quasars and compact galaxies predicted 
to be found with the Rubin and Roman telescopic surveys could reach 10 thousand systems. Obtaining precision astrometry for the full sample is likely out of the question.
Thus, to fully leverage the sample of lensed systems for the measurement of cosmological 
parallax would require some portion of the time on dedicated ELTs located in both the northern and the southern hemispheres. 
While expensive, this strategy would also result in constraints on the Dark Energy equation of state 
that are as much as 10x higher precision than those currently available from BAO or SNIa. 
A lower precision measurement could be accomplished over a shorter baseline, 
perhaps in only a few years, with the signal growing 
with time. We also note that significant developmental savings in 
costs and time could be accomplished by copying the designs of either the Giant Magellan or 
the Thirty Meter Telescopes, their adaptive optics systems and limiting their suite of 
instrumentation.
 
The precision astrometry we are proposing for even the largest samples would require about 
10\% of the time available on an ELT, meaning that the remainder of the time could be dedicated 
to other precision cosmological measurements. The narrow-fields of the ELTs likely precludes 
their use in the next generation large-scale spectroscopic surveys that are being 
proposed elsewhere in this document but they would naturally be applicable to direct measures 
of cosmic deceleration.

%\end{document}

